Sketch-Guided Constrained Decoding for Boosting Blackbox Large Language Models without Logit Access

Constrained decoding, a technique for enforcing constraints on language model outputs, offers a way to control text generation without retraining or architectural modifications. Its application is, however, typically restricted to models that give users access to next-token distributions (usually via softmax logits), which poses a limitation with blackbox large language models (LLMs). This paper introduces sketch-guided constrained decoding (SGCD), a novel approach to constrained decoding for blackbox LLMs, which operates without access to the logits of the blackbox LLM. SGCD utilizes a locally hosted auxiliary model to refine the output of an unconstrained blackbox LLM, effectively treating this initial output as a "sketch" for further elaboration. This approach is complementary to traditional logit-based techniques and enables the application of constrained decoding in settings where full model transparency is unavailable. We demonstrate the efficacy of SGCD through experiments in closed information extraction and constituency parsing, showing how it enhances the utility and flexibility of blackbox LLMs for complex NLP tasks.

==> sections/09_contribution.tex <==
\xhdr{Contributions}
Our work makes the following contributions to the field:

\begin{itemize}
    \denselist
    \item We propose a novel method for applying constraints to the output of \blackbox{} LLMs without direct access to the model's logits, which largely expands the scope of constrained decoding methods.
    \item We demonstrate that \ourmethod{} can be effectively implemented using smaller models that are feasible for operation on standard consumer hardware, while still leveraging the advanced capabilities of larger LLMs hosted remotely.
    \item Through extensive experiments and evaluations, we establish that \ourmethod{} can significantly boost the performance LLMs and beat previous approaches by a large margin.
\end{itemize}

==> tables/IE_SGCD_Q_VS_A.tex <==
\begin{table*}[tb]
\centering
\resizebox{0.8\textwidth}{!}{
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}llll|lll@{}}
\toprule
& \multicolumn{3}{c}{Wiki-NRE} & \multicolumn{3}{c}{SynthIE-text}  \\
& Precision & Recall & F1 & Precision & Recall & F1  \\
\midrule
\hspace{4mm} \GPTfour{}                &   &      &       &        &     &      \\
\rowcolor{lightblue}
%\textbf{\hspace{4mm} \GPTfour{} + \ourmethod{}}     &    56.9{\scriptsize±  3.2}     &    47.4{\scriptsize±  2.9}     &    48.6{\scriptsize±  2.8}    &    50.3{\scriptsize±  2.5}     &  41.0{\scriptsize±  2.3}     &    43.4{\scriptsize±  2.2}    \\
\textbf{\hspace{8mm}  +\ourmethod{}(Lossy)} &   xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xxx}   &  xxx{\scriptsize±  xxx}     &  xxx{\scriptsize±  xxx}     &    xxx{\scriptsize±  xxx}    \\
\textbf{\hspace{8mm}  +\ourmethod{}} &   xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xxx}   &  xxx{\scriptsize±  xxx}     &  xxx{\scriptsize±  xxx}     &    xxx{\scriptsize±  xxx}    \\
\hspace{4mm} \llama-2-70B                    &   &      &       &        &     &      \\
\rowcolor{lightblue}
\textbf{\hspace{8mm}  +\ourmethod{}(Lossy)} &   xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xxx}   &  xxx{\scriptsize±  xxx}     &  xxx{\scriptsize±  xxx}     &    xxx{\scriptsize±  xxx}    \\
%\textbf{\hspace{4mm} \GPTthreeFiveTurbo{} + \ourmethod{}}   &    47.6{\scriptsize±  3.3}     &    37.9{\scriptsize±  2.8}     &    39.4{\scriptsize±  2.8}   &    44.2{\scriptsize±  2.8}     &  32.4{\scriptsize±  2.1}     &    35.3{\scriptsize±  2.1}     \\
\textbf{\hspace{8mm}  +\ourmethod{}} &   xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xxx}   &  xxx{\scriptsize±  xxx}     &  xxx{\scriptsize±  xxx}     &    xxx{\scriptsize±  xxx}    \\
\hspace{4mm} \llama-33B                     &   &      &       &        &     &      \\
\rowcolor{lightblue}
\textbf{\hspace{8mm}  +\ourmethod{}(Lossy)} &   xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xxx}   &  xxx{\scriptsize±  xxx}     &  xxx{\scriptsize±  xxx}     &    xxx{\scriptsize±  xxx}    \\
%\textbf{\hspace{4mm} Claude + \ourmethod{}}      &    49.4{\scriptsize±  2.5}    &    37.5{\scriptsize±  2.8}     &    40.3{\scriptsize±  2.9}   &   46.2{\scriptsize±  2.5}     &  35.8{\scriptsize±  2.2}     &    38.3{\scriptsize±  2.2}     \\
\textbf{\hspace{8mm}  +\ourmethod{}} &   xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xxx}   &  xxx{\scriptsize±  xxx}     &  xxx{\scriptsize±  xxx}     &    xxx{\scriptsize±  xxx}    \\
\hspace{4mm} \llama-2-13B              &   &      &       &        &     &      \\
\rowcolor{lightblue}
\textbf{\hspace{8mm}  +\ourmethod{}(Lossy)} &   xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xxx}   &  xxx{\scriptsize±  xxx}     &  xxx{\scriptsize±  xxx}     &    xxx{\scriptsize±  xxx}    \\
%\textbf{\hspace{4mm} Claude-instant + \ourmethod{}} &   39.6{\scriptsize±  3.3}       &    29.6{\scriptsize±  2.7}     &    31.9{\scriptsize±  2.5}   &   37.8{\scriptsize±  2.6}     &  27.2{\scriptsize±  2.1}     &  30.0{\scriptsize±  2.1}  \\
\textbf{\hspace{8mm}  +\ourmethod{}} &   \textbf{39.6{\scriptsize±  3.3} }       &    \textbf{29.6{\scriptsize±  2.7}}     &    \textbf{31.9{\scriptsize±  2.5}}   &   \textbf{37.8{\scriptsize±  2.6} }     &  \textbf{27.2{\scriptsize±  2.1} }     &  \textbf{30.0{\scriptsize±  2.1} }  \\
%\hspace{4mm} PaLM-2-text         &  19.1{\scriptsize±  1.9}    &  23.0{\scriptsize±  2.4}     &  19.9{\scriptsize±  2.0}   &  28.1{\scriptsize±  2.1}     &  26.7{\scriptsize±  2.0}     &    27.1{\scriptsize±  2.0}    \\
\rowcolor{lightblue}
\hspace{4mm} \llama-2-7B              &   &      &       &        &     &      \\
\rowcolor{lightblue}
\textbf{\hspace{8mm}  +\ourmethod{}(Lossy)} &   xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xx}     &    xxx{\scriptsize±  xxx}   &  xxx{\scriptsize±  xxx}     &  xxx{\scriptsize±  xxx}     &    xxx{\scriptsize±  xxx}    \\
%\textbf{\hspace{4mm} Claude-instant + \ourmethod{}} &   39.6{\scriptsize±  3.3}       &    29.6{\scriptsize±  2.7}     &    31.9{\scriptsize±  2.5}   &   37.8{\scriptsize±  2.6}     &  27.2{\scriptsize±  2.1}     &  30.0{\scriptsize±  2.1}  \\
\textbf{\hspace{8mm}  +\ourmethod{}} &   \textbf{39.6{\scriptsize±  3.3} }       &    \textbf{29.6{\scriptsize±  2.7}}     &    \textbf{31.9{\scriptsize±  2.5}}   &   \textbf{37.8{\scriptsize±  2.6} }     &  \textbf{27.2{\scriptsize±  2.1} }     &  \textbf{30.0{\scriptsize±  2.1} }  \\
%\hspace{4mm} PaLM-2-text         &  19.1{\scriptsize±  1.9}    &  23.0{\scriptsize±  2.4}     &  19.9{\scriptsize±  2.0}   &  28.1{\scriptsize±  2.1}     &  26.7{\scriptsize±  2.0}     &    27.1{\scriptsize±  2.0}    \\
\rowcolor{lightblue}\bottomrule
\end{tabular}
}
% Saibo Version
%\caption{\textbf{Main results for closed information extraction (4 shots),} in terms of triplet-based precision, recall, and F1-score (micro-averaged, with 90\% confidence intervals) on the Wiki-NRE and SynthIE-text datasets.
%\ourmethod{} uses \llama-7B as the constraint model. CD stands for constrained decoding.
%}
\caption{\textbf{Results for closed information extraction,} in terms of triplet-based precision, recall, and F1-score (micro-averaged, with bootstrapped 95\% confidence intervals) on the Wiki-NRE and SynthIE-text datasets. The results compare the effectiveness of \ourmethod{} (blue rows) against two baselines:
(1) few-shot-prompted unconstrained decoding with powerful \blackbox{} LLMs (``without logit access'', white rows, \Eqnref{eq:sketching}) and
(2) few-shot-prompted constrained decoding (``CD'') with \opensourceLLMs{} (``with logit access'', \Eqnref{eq:constrained_generation}).
Four demonstrations are used in few-shot prompting.
\llama-7B serves as the constrained generator $P_\text{cg}$ for \ourmethod{}.}
\label{tab:InformationExtractionResults}
\end{table*}



